Variable Elimination in the Fourier Domain

The ability to represent complex high dimensional probability distributions in a compact form is one of the key insights in the field of graphical models. Factored representations are ubiquitous in machine learning and lead to major computational advantages. We explore a different type of compact representation based on discrete Fourier representations, complementing the classical approach based on conditional independencies. We show that a large class of probabilistic graphical models have a compact Fourier representation. This theoretical result opens up an entirely new way of approximating a probability distribution. We demonstrate the significance of this approach by applying it to the variable elimination algorithm. Compared with the traditional bucket representation and other approximate inference algorithms, we obtain significant improvements.

==> Makefile <==
.PHONY: main fromscratch dvi ps pdf bibs xfigs compact clean tar tgz

TEXFILE    = fourier_icml16

LATEX      = latex
BIBTEX     = bibtex
MAKEINDEX  = makeindex
DVIPS      = dvips -t letter
PDFLATEX   = pdflatex
PS2PDF     = ps2pdf
XFIGDIR     = xfigs
CURRENTDIR = `basename "\`pwd\`"`

default: pdf

#fromscratch: xfigs
fromscratch:
	$(LATEX) $(TEXFILE)
	$(BIBTEX) $(TEXFILE)
	$(LATEX) $(TEXFILE)
	$(LATEX) $(TEXFILE)
	$(DVIPS) $(TEXFILE).dvi -o $(TEXFILE).ps

dvi:
	$(LATEX) $(TEXFILE)

ps: dvi
	$(DVIPS) $(TEXFILE).dvi -o $(TEXFILE).ps

pdf:
	# $(LATEX) $(TEXFILE)
	# $(BIBTEX) $(TEXFILE)
	# $(LATEX) $(TEXFILE)
	# $(LATEX) $(TEXFILE)
	$(PDFLATEX) $(TEXFILE)
	$(BIBTEX) $(TEXFILE)
	$(PDFLATEX) $(TEXFILE)
	$(PDFLATEX) $(TEXFILE)
#pdf: ps
#$(PS2PDF) $(TEXFILE)

bibs:
	$(BIBTEX) $(TEXFILE)

xfigs:
	(cd $(FIGDIR); bash ./makefigs ../*.tex )

compact:
#	(rm -f *.aux *.log *.blg *.out *.toc $(TEXFILE).bbl)
	(rm -f *.aux *.log *.blg *.out *.toc)

clean: compact
#	(rm -f *.dvi *.ps *.pdf $(FIGDIR)/*.{eps,pdf,pstex,pstex_t,fig.bak} )
	(rm -f *.dvi *.ps *.pdf $(TEXFILE).bbl $(FIGDIR)/*.{eps,pdf,pstex,pstex_t,fig.bak} )

tar:
	rm -f ../$(CURRENTDIR).tar.gz
	tar cvf ../$(CURRENTDIR).tar ../$(CURRENTDIR)
	gzip ../$(CURRENTDIR).tar
	echo "Created ../$(CURRENTDIR).tar.gz"

tgz:
	rm -f ../$(CURRENTDIR).tgz
	tar cvfz ../$(CURRENTDIR).tgz ../$(CURRENTDIR)
	echo "Created ../$(CURRENTDIR).tgz"



==> supply/Makefile <==
.PHONY: main fromscratch dvi ps pdf bibs xfigs compact clean tar tgz

TEXFILE    = icml16_supply

LATEX      = latex
BIBTEX     = bibtex
MAKEINDEX  = makeindex
DVIPS      = dvips -t letter
PDFLATEX   = pdflatex
PS2PDF     = ps2pdf
XFIGDIR     = xfigs
CURRENTDIR = `basename "\`pwd\`"`

default: pdf

#fromscratch: xfigs
fromscratch:
	$(LATEX) $(TEXFILE)
	$(BIBTEX) $(TEXFILE)
	$(LATEX) $(TEXFILE)
	$(LATEX) $(TEXFILE)
	$(DVIPS) $(TEXFILE).dvi -o $(TEXFILE).ps

dvi:
	$(LATEX) $(TEXFILE)

ps: dvi
	$(DVIPS) $(TEXFILE).dvi -o $(TEXFILE).ps

pdf:
	# $(LATEX) $(TEXFILE)
	# $(BIBTEX) $(TEXFILE)
	# $(LATEX) $(TEXFILE)
	# $(LATEX) $(TEXFILE)
	$(PDFLATEX) $(TEXFILE)
#	$(BIBTEX) $(TEXFILE)
	$(PDFLATEX) $(TEXFILE)
	$(PDFLATEX) $(TEXFILE)
#pdf: ps
#$(PS2PDF) $(TEXFILE)

bibs:
	$(BIBTEX) $(TEXFILE)

xfigs:
	(cd $(FIGDIR); bash ./makefigs ../*.tex )

compact:
#	(rm -f *.aux *.log *.blg *.out *.toc $(TEXFILE).bbl)
	(rm -f *.aux *.log *.blg *.out *.toc)

clean: compact
#	(rm -f *.dvi *.ps *.pdf $(FIGDIR)/*.{eps,pdf,pstex,pstex_t,fig.bak} )
	(rm -f *.dvi *.ps *.pdf $(TEXFILE).bbl $(FIGDIR)/*.{eps,pdf,pstex,pstex_t,fig.bak} )

tar:
	rm -f ../$(CURRENTDIR).tar.gz
	tar cvf ../$(CURRENTDIR).tar ../$(CURRENTDIR)
	gzip ../$(CURRENTDIR).tar
	echo "Created ../$(CURRENTDIR).tar.gz"

tgz:
	rm -f ../$(CURRENTDIR).tgz
	tar cvfz ../$(CURRENTDIR).tgz ../$(CURRENTDIR)
	echo "Created ../$(CURRENTDIR).tgz"



==> supply/theory_supply.tex <==
\section{Proof of Lemma 1}


Let $R_n^l$ be the collection of restrictions on $n$ Boolean variables
$x_1, \ldots, x_n$. Each restriction in $R_n^l$ leaves a set of $l$ variables $J=\{x_{i_1}, \ldots, x_{i_l}\}$ open, while it fixes all other
variables $x_i \not \in J$ to either -1 or 1. It is easy to see
that the size of $R_n^l$ is given by:
\begin{equation}
  |R_n^l| = {n \choose l} \cdot 2^{n-l}.
\end{equation}

For a restriction $J|\z \in R_n^l$, call $J|\z$ \textit{bad} if and
only if for all decision tree $h$ with depth $t$, there exists at
least one input $\x_J$, such that $|h(\x_J) - f|_{J|\z}(\x_J)| >
\gamma$. Let $B_n^l$ be the set of all bad restrictions, ie: 
$B_n^l = \{J|\z \in R_n^l: J|\z \mbox{ is bad}\}$. 
%
To prove the lemma, it is sufficient to prove that 
\begin{equation}
  \frac{|B_n^l|}{|R_n^l|} \leq \frac{1}{2} \left(\frac{l}{n-l} 8 u w\right)^t. 
\end{equation}

In the proof that follows, for every bad restriction $\rho \in B_n^l$,
we establish a bijection between $\rho$ and $(\xi, s)$, in which $\xi$
is a restriction in $R_n^{l-t}$ and $s$ is a certificate from a
witness set $A$. In this case, the number of distinct $\rho$'s is
bounded by the number of $(\xi, s)$ pairs: %. In other words,
\begin{equation}
  |B_n^l| \leq |R_n^{l-t}| \cdot |A|.
\end{equation}

For a restriction $\rho$, we form the \textit{canonical decision
 tree} for $f|_\rho$ under precision $\gamma$ as follows: 
\begin{enumerate}
\item We start with a fixed order for the
  variables and another fixed order for the factors. 
%Then we examine the factors in this fixed order. 
\item If $f|_\rho$ is a constant function, or $||f|_\rho||_\infty \leq
  \gamma$, stop.
%
\item Otherwise, under restriction $\rho$, some factors evaluate to
  fixed values (all variables in these factors are fixed or there are
  free variables, but all assignments to these free variables lead to
  value 1), while other factors do not.  Examine the factors according
  to the fixed factor order until reaching the first factor that still
  does not evaluate to a fixed value.
%
\item Expand the open variables of this factor, under the fixed
  variable order specified in step 1. The result will be a tree (The
  root branch is for the first open variable. The branches in the
  next level is for the second open variable, etc).
%
\item Each leaf of this tree corresponds to $f|_{\rho\pi_1}$, in
  which $\pi_1$ is a value restriction for all open variables of the
  factor. Recursively apply step 2 to 5 for function
  $f|_{\rho\pi_1}$, until the condition in step 2 holds. Then attach
  the resulting tree to this leaf.
\end{enumerate}

Figure~\ref{fig:decision_tree} provides a graphical demonstration of a
canonical decision tree.

Now suppose restriction $\rho$ is bad. By definition, for any decision
tree of depth $t$, there exists at least one input $\x$, such that
$|h(\x) - f|_{\rho}(\x)| > \gamma$.
%
The canonical decision tree is no exception. Therefore, there must be
a path $l$ in the canonical decision tree of $f|_\rho$, which has more
than $t$ variables. Furthermore, these $t$ variables can be split into
$k$ ($1\leq k \leq t$) segments, each of which corresponds to one
factor.
%
Let $f_i$ ($i\in\{1,\dots,k\}$) be these factors, and let $\pi_i$ be
the assignments of the free variables for $f_i$ in path $l$. 
%
Now for each factor $f_i$, by the definition of the canonical decision
tree, under the restriction $\rho\pi_1\dots\pi_{i-1}$,
$f_i|\rho\pi_1\dots\pi_{i-1}$ must have a branch whose value is no
greater than $\eta$ (otherwise $f_i|\rho\pi_1\dots\pi_{i-1}$ all
evaluates to 1). We call this branch the ``compressing'' branch for factor $f_i|\rho\pi_1\dots\pi_{i-1}$. 
%
Let the variable assignment which leads to this compressing branch for
$f_i|\rho\pi_1\dots\pi_{i-1}$ be $\sigma_i$. Let $\sigma = \sigma_1
\ldots \sigma_k$. Then we map the bad restriction $\rho$ to $\rho
\sigma$ and an auxiliary advice string that we are going to describe.
\begin{figure}
  \centering
  \includegraphics[width=0.9\linewidth]{canonical_decision_tree}
  \caption{A graphical illustration of a canonical decision tree.}
  \label{fig:decision_tree}
\end{figure}

It is self-explanatory that we can map from any bad restriction $\rho$
to $\rho \sigma$. The auxiliary advice is used to establish the
backward mapping, i.e. the mapping from $\rho\sigma$ to $\rho$.
%
When we look at the result of $f|\rho\sigma$, we will notice that at
least one factor is set to its compressing branch (because we set
$f_1$ to its compressing branch in the forward mapping). 
%
Now there could be other factors set at their compressing branches
(because of $\rho$), but an important observation is that: \textit{the
  number of factors at their compressing branches cannot exceed
  $u=\lceil \log_\eta \gamma \rceil+1$}, because otherwise, the other
$u-1$ factors already render $||f|\rho||_\infty \leq \gamma$, and the
canonical decision tree should have stopped on expanding this branch.
%
We therefore could record the index number of $f_1$ out of all the
factors that are fixed at their compressing branches in the auxiliary
advice string, so we can find $f_1$ in the backward mapping. Notice
that this index number will be between 1 and $u$, so it takes $\log u$
bits to store it.

Now with the auxiliary information, we can identify which factor is
$f_1$. The next task is to identify which variables in $f_1$ are fixed
by $\rho$, and which are fixed by $\sigma_1$. Moreover, if one
variable is fixed by $\sigma_1$, we would like to know its correct
values in $\pi_1$. To do this, we introduce additional auxiliary
information: for each factor $f_i$, suppose it has $r_i$ free
variables under restriction $f_i|\rho\pi_1\dots\pi_{i-1}$, we use
$r_i$ integers to mark the indices of these free variables. Because each $f_i$ is of width at most $w$, every integer of this type is between 1 and $w$ (therefore can be stored in $\log w$ bits). Also, it requires $t$ integers of this type in total to keep this
information, because we have $t$ free variables in total for $f_1,
\ldots, f_k$.
%
%% , each of which . 

Notice that it is not sufficient to keep these integers. We further
need $k-1$ separators, which tell which integer belongs to which factor 
$f_i$. Aligning these integers in a line, we need $k-1$ separators to
break the line into $k$ segments. These separators can be represented
by $t-1$ bits, in which the $i$-th bit is 1 if and only if there is a
separator between the $i$-th and ($i$+1)-th integer (we have $t$
integers at most).
%
With these two pieces of information, we are able to know the locations of free variables set by $\sigma_i$ for each factor $f_i$.

We further need to know the values for each variable in
$\pi_i$. Therefore, we add in another $t$-bit string, each bit is
either 0 or 1. 0 means the assignment of the corresponding variable in
$\pi_i$ is the same as the one in $\sigma_i$, 1 means the opposite.

With all this auxiliary information, we can start from $\rho \sigma$,
find the first factor $f_1$, further identify which variables are set
by $\sigma_1$ in $f_1$, and set back its values in $\pi_1$. Then we
start with $f|\pi_1$, we can find $\pi_2$ in the same process, and
continue. Finally, we will find all variables in $\sigma$ and back up
the original restriction $\rho$.

Now to count the length of the auxiliary information, the total length
is $t\log u + t\log w + 2t - 1$ bits. Therefore, we can have a
one-to-one mapping between elements in $B_n^l$ and $R_n^{l-t} \times
A$, in which the size of $A$ is bounded by $2^{t\log u + t\log w + 2t
  - 1} = (uw)^t \cdot 2^{2t-1}$.

In all, 
\begin{align}
  \frac{|B_n^l|}{|R_n^l|} &\leq \frac{{n \choose l-t} 2^{n-l+t} (uw)^t \cdot 2^{2t-1}}{{n \choose l} 2^{n-l}}\\
  &=\frac{{n \choose l-t} \frac{1}{2} (8uw)^t }{{n \choose l} }\\
  &=\frac{l(l-1)\ldots(l-t+1)}{(n-l+1)\ldots(n-l+t)} \frac{1}{2}(8uw)^t\\
  &\leq \frac{1}{2} \left(\frac{l}{n-l} 8 u w\right)^t. 
\end{align}

\section{Proof of Theorem 3}

For each term in the Fourier expansion whose degree is less than or equal to $d$, we can treat this term as a weighted function involving less than or equal to $d$ variables. Therefore, it can be represented by a decision tree, in which each path of the tree involves no more than $d$ variables (therefore the tree is at most at the depth of $d$). Because $f$ is represented as the sum over a set of Fourier terms up to degree $d$, it can be also represented as the sum of the corresponding decision trees. 

\section{Proof of Theorem 6}
%% Because the Fourier coefficient is connected with its function values through an expectation:
%% $$\hat{f}(S) = \mathbb{E}_{\x} \left( f(\x) \chi_S(\x) \right).$$
%% For $f'(\x \setminus x_0) =\sum_{x_0} f(\x \setminus x_0, x_0) = f(\x \setminus x_0, x_0=+1) + f(\x \setminus x_0, x_0=-1)$, when $x_0 \in S$, 
%% $$f(\x \setminus x_0, x_0=+1) \chi_S(\x) = f(\x \setminus x_0, x_0=+1) \chi_S(\x \setminus x_0) \cdot x0 $$

Let the Fourier expansion of $f$ be: $f(\x)= \sum_S \hat{f}(S) \chi_S(\x)$, we have: 
\begin{align*}
&f'(\x \setminus x_i)\\
=&f(\x \setminus x_i, x_i=+1) + f(\x \setminus x_i, x_i=-1)\\
=&\sum_{S: i \in S} \hat{f}(S) \cdot \chi_{S\setminus i}(\x \setminus x_i) \cdot 1+\\
 &\sum_{S: i \not \in S} \hat{f}(S) \cdot \chi_{S\setminus i}(\x \setminus x_i)  \\
&  + \sum_{S: i \in S} \hat{f}(S) \cdot \chi_{S\setminus i}(\x \setminus x_i) \cdot (-1) + \\
 &\sum_{S: i \not \in S} \hat{f}(S) \cdot \chi_{S\setminus i}(\x \setminus x_i)\\
=&\sum_{S: i \in S} \hat{f}(S) \cdot \chi_{S\setminus i}(\x \setminus x_i) \cdot 1 + \\
&\sum_{S: i \in S} \hat{f}(S) \cdot \chi_{S\setminus i}(\x \setminus x_i) \cdot (-1)  \\
& + \sum_{S: i \not \in S} \hat{f}(S) \cdot \chi_{S\setminus i}(\x \setminus x_i) + \\
&\sum_{S: i \not \in S} \hat{f}(S) \cdot \chi_{S\setminus i}(\x \setminus x_i)\\
=& \sum_{S: i \not \in S} 2 \cdot \hat{f}(S) \cdot \chi_{S\setminus i}(\x \setminus x_i).
\end{align*}

